Challenges for variational reduced-density-matrix theory: Total angular momentum constraints

The variational two-electron reduced density matrix (v2RDM) method is generalized for the description of total angular momentum ($J$) and projection of total angular momentum ($M_{J}$) states in atomic systems described by non-relativistic Hamiltonians, and it is shown that the approach exhibits serious deficiencies. Under ensemble $N$-representability constraints, v2RDM theory fails to retain the appropriate degeneracies among various $J$ states for fixed spin ($S$) and orbital angular momentum ($L$), and, for fixed $L$, $S$, and $J$, the manifold of $M_{J}$ states are not necessarily degenerate. Moreover, a substantial energy error is observed for a system for which the two-electron reduced density matrix is exactly ensemble $N$-representable; in this case, the error stems from violations in pure-state $N$-representability conditions. Unfortunately, such violations do not appear to be good indicators of the reliability of energies from v2RDM theory in general. Several states are identified for which energy errors are near zero and yet pure-state conditions are clearly violated.

==> discussion_revision.tex <==
Before moving on, we highlight two subtle yet important differences between v2RDM calculations that place constraints on $S$, $L$, $M_L$, and $M_S$ versus those that place constraints on $S$, $L$, $J$, and $M_J$. We refer to these cases as uncoupled and coupled angular momentum states, respectively. First, for uncoupled states, we preserve the spin-blocked structure expected for RDMs that derive from wave functions having good spin-projection quantum numbers, whereas this block structure is relaxed for coupled states. Figure \ref{FIG:C_3P_L} provides errors in v2RDM-derived energies for ${}^3$P spin and orbital angular momentum projection states of a carbon atom. Here, results labeled ``spin blocks'' and ``no spin blocks'' correspond to calculations performed under the PQG conditions, with constraints on the expectation values of $\hat{L}^2$, $\hat{S}^2$, $\hat{L}_z$, and $\hat{S}_z$, as well as constraints on the variances of $\hat{L}_z$ and $\hat{S}_z$; the only difference between the calculations is the block structure imposed on the RDMs. We can see that, for maximal spin projections ($M_S$ = $\pm 1$), different orbital angular momentum projection states are degenerate, regardless of the block structure of the RDMs. On the other hand, both sets of calculations fail to retain the correct degeneracy in the orbital angular momentum projection states when $M_S = 0$, and worse results are obtained for the case that relaxes the spin block structure. Hence, we can conclude that the additional variational flexibility introduced via the relaxed spin block structure in coupled angular momentum calculations exaggerates the existing  degeneracy issues in the uncoupled case.

\begin{figure}
    \caption{Errors in v2RDM-derived energies of $^3$P spin and orbital angular momentum projection states of a carbon atom. }
    \label{FIG:C_3P_L}
    \begin{center}
        \includegraphics[scale=1.0]{figures/C_3P_L.eps}
    \end{center}
\end{figure}

The second difference between v2RDM calculations describing uncoupled and coupled angular momentum states is that the states themselves are different; coupled angular momentum states are admixtures of uncoupled states, as defined by the Wigner--Eckart theorem. Figure \ref{FIG:B_2P_CG} illustrates errors in v2RDM-derived energies for the ${}^2$P states of a boron atom, and the schematic connects coupled angular momentum states to the uncoupled states to which they should correspond. Here, calculations on uncoupled and coupled states both consider RDMs that satisfy the PQG conditions. Uncoupled calculations consider constraints on $S^2$, $L^2$, $M_S$, and $M_L$, while coupled calculations consider constraints on $S^2$, $L^2$, $J^2$, and $M_J$. Neither set of calculations imposes spin-block structure on the RDMs so that we can focus on the angular momentum constraints themselves. In this case, we find that the energies of uncoupled states are well-described by v2RDM theory and that the approached exhibits no degeneracy issues. On the other hand, coupled states are not degenerate, and  the correct energy is only obtained for the maximal $J$ state with $M_J = J$. The data in Fig.~\ref{FIG:B_2P_CG} suggest that the energies of coupled angular momentum states are a lower bound to those of uncoupled states, but this is not actually the case, in general. A similar analysis for the $^3$P state of carbon can be found in the Supporting Information; in this case, some coupled states lie higher in energy than the parent uncoupled states.


\begin{figure}
    \caption{Errors in v2RDM-derived energies for various $^2$P angular momentum states of a boron atom.}
    \label{FIG:B_2P_CG}
    \begin{center}
        \includegraphics[scale=1.0]{figures/B_2P_CG_diagram.eps}
    \end{center}
\end{figure}


\subsection{Ensemble- versus pure-state $N$-representability}
\label{SEC:GPC}

All v2RDM-derived results presented in this work were generated under ensemble $N$-representability conditions. In this Section, we draw connections between the degeneracy issues discussed above and violations in pure-state conditions not enforced in our calculations. A useful case study for this purpose is the ${}^1$P$_1$ state of atomic beryllium. Moving forward, for v2RDM calculations on this system and for all remaining v2RDM optimizations, we enforce constraints on the expectation values of $\hat{S}^2$, $\hat{L}^2$, $\hat{J}^2$, and $\hat{J}_z$, as well as on the variance of $\hat{J}_z$. Table \ref{TABLE:BE_1P1} provides errors in energies from v2RDM calculations where RDMs satisfied the PQG or PQG plus T2 constraints, as compared to results taken from full CI calculations. While PQG constraints lead to accurate energies for the maximal projections ($M_J = \pm 1$), these constraints do not provide a good description of the $M_J = 0$ state. In this case, v2RDM energies are 0.1679 E$_{\rm h}$ too low. Moreover, the addition of the T2 constraint only improves the energy by 0.0001 E$_{\rm h}$. This failure comes as a surprise, as Be only has two valence electrons, so one would expect that PQG constraints should provide an accurate description of its electronic structure, as in the case of the maximal projection states tabulated in Table \ref{TABLE:BE_1P1}.


\begin{table}[]
\caption{Errors in v2RDM-derived energies (10$^{-3}$ E$_{\rm h}$) for different total angular momentum projections of the ${}^1$P$_1$ state of beryllium.}
\label{TABLE:BE_1P1}
\begin{tabular}{ccdd}
\hline\hline
$M_J$ &~& \multicolumn{1}{c}{PQG}  & \multicolumn{1}{c}{PQGT2} \\
\hline
-1 &~&     0.0  &    0.0  \\
0  &~&  -167.9  & -167.8  \\
1  &~&     0.0  &    0.0  \\
\hline\hline             
\end{tabular}
\end{table}

\subsubsection{Generalized Pauli constraints for the $^{1}$P$_1$ state of beryllium}

While necessary ensemble $N$-representability conditions on $p$-body RDMs are straightforward to devise,\cite{Erdahl01_042113} and a complete solution to the ensemble $N$-representability problem has been put forward,\cite{Mazziotti12_263002} the pure-state $N$-representability problem is much more complex. Indeed, until only a short while ago,\cite{Klyachko06_72,Klyachko08_287} necessary and sufficient pure-state conditions on the 1RDM, known as generalized Pauli constraints (GPCs), were only known for special cases.\cite{Dennis72_7} \textcolor{black}{The GPCs are sets of constraints on the natural orbital occupation numbers. } In Ref.~\citenum{Klyachko08_287}, however, Altunbulak and Klyachko developed an algorithm to identify GPCs for general systems and tabulated these constraints for systems involving up to ten spin orbitals. These GPCs also indirectly apply to the 2RDM.\cite{Mazziotti16_032516} As shown in the Appendix, GPCs can be applied to the 1RDM for $(N-1)$- or $(N+1)$-electron systems generated by the removal or addition of an electron to the $N$-electron state, respectively; such constraints can be expressed in terms of the 2RDM for the $N$-electron state. Enforcing GPCs can be challenging, in practice.\cite{DePrince16_164109, Helbig15_154108} In this work, we merely assess whether 1RDMs and 2RDMs optimized under ensemble $N$-representability constraints satisfy these conditions. \textcolor{black}{For each system, whenever a GPC constraint is violated, the amount of the violations is summed into the GPC error, presented in Tables 2, 3, and 5. The unit of the violations is number of electrons.}

We begin with the troubling case of the ${}^1$P$_1$ state of beryllium, as described by v2RDM calculations that enforce the PQG constraints, within STO-3G basis set. The family of antisymmetrized wave functions corresponding to this four electron / ten spin orbital system is represented by the symbol  $\wedge^4\mathcal{H}_{10}$. 
Table \ref{TABLE:Be_FULL_GPC} provides the energy error and GPC errors for the $M_J = 0$ and $M_J = 1$ projections of the ${}^1$P$_1$ state. The errors are defined as the sum of all violated GPCs, and a negative value indicates that the conditions are violated. The notation $N-1$ and $N+1$ refer to GPCs applied to the 1RDM for the $(N-1)$- or $(N+1)$-electron states, respectively,
and wave functions for these systems belong to the $\wedge^3\mathcal{H}_{10}$ and $\wedge^5\mathcal{H}_{10}$ families, respectively. 
We note that the $(N \pm 1)$-electron wave functions are defined by the expansions given in the Appendix (see Eqs.~\ref{EQN:NM1_STATE} and \ref{EQN:NP1_STATE}, respectively), with the expansion coefficients assumed to be real and chosen to maximize the magnitude of the errors in the GPCs (see the Appendix for a more detailed description of this procedure). As mentioned above, such conditions actually apply to the 2RDM for the $N$-electron state. From these data, we first note that the GPCs on the 1RDM for the $N$-electron state are satisfied. However, GPCs applied to the 2RDM are violated for both projections, with the larger errors observed for the $M_J = 0$ case (the case for which the energy is poorly described by ensemble conditions). Hence, it appears that large energy errors are associated with violations in GPCs on the 2RDM, but the converse cannot be stated. A small energy error does not guarantee that the GPCs on the 2RDM are necessarily satisfied. 

\begin{table}[]
\centering
\caption{Energy errors (10$^{-3}$ E$_{\rm h}$) and GPC errors for the $M_J = 0$ and $M_J = 1$ projections of the ${}^1$P$_1$ state of beryllium. The full CI and v2RDM calculations correlated all four electrons in all ten spin orbitals. }
\label{TABLE:Be_FULL_GPC}
\begin{tabular}{ccdddd}
\hline
\hline
 & & & \multicolumn{3}{c}{GPC errors} \\
 \cline{4-6}
 & & &      & \multicolumn{2}{c}{2RDM} \\
 \cline{5-6}
 & $M_J$ & \multicolumn{1}{c}{energy error} & \multicolumn{1}{c}{1RDM} & \multicolumn{1}{c}{$N-1$} & \multicolumn{1}{c}{$N+1$} \\
\hline
${}^1$P$_1$ & 0 & -167.9 & 0.00 & -350.86 & -91.34 \\
${}^1$P$_1$ & 1 & 0.0 & 0.00 & -22.62 & 0.00 \\
                               \hline\hline
\end{tabular}
\end{table}

Given the large violations in the GPCs on the 2RDM tabulated in Table \ref{TABLE:Be_FULL_GPC}, it is interesting to consider the same states, but for the case where we do not correlate the electrons in the 1s orbital. This situation corresponds to an active-space v2RDM calculation on two electrons in eight spin orbitals, and the PQG constraints are complete ensemble $N$-representability conditions in this case. Table \ref{TABLE:Be_GPC} provides the energy error and GPC errors for the $M_J = 0$ and $M_J = 1$ projections of the ${}^1$P$_1$ state, with the 1s electrons frozen. The results for the $M_J = 1$ state are unsurprising; the energy error is zero, and the GPCs on the 1RDM and 2RDM are all satisfied. However, the error in the v2RDM energy for the $M_J = 0$ state is almost as large as that for the full space calculation (-0.1675 E$_{\rm h}$, as compared to the energy from an active space full CI calculation with the same active space), despite the fact that the v2RDM-optimized 1RDM and 2RDM are \textit{exactly} ensemble $N$-representable. In this case, we find that GPCs on the 1RDM are satisfied, as are the GPCs on the 1RDM for the ($N-1$)-electron state. On the other hand, the GPCs on the 1RDM for the ($N+1$)-electron state are violated, and we can thus conclude that the energy error is related to the ensemble nature of the 2RDM.


\begin{table}[]
\centering
\caption{Energy errors (10$^{-3}$ E$_{\rm h}$) and GPC errors for the $M_J = 0$ and $M_J = 1$ projections of the ${}^1$P$_1$ state of beryllium. The full CI and v2RDM calculations correlated an active space of two electrons in eight spin orbitals. }
\label{TABLE:Be_GPC}
\begin{tabular}{ccdddd}
\hline
\hline
 & & & \multicolumn{3}{c}{GPC errors} \\
 \cline{4-6}
 & & &      & \multicolumn{2}{c}{2RDM} \\
 \cline{5-6}
  & $M_J$ & \multicolumn{1}{c}{energy error} & \multicolumn{1}{c}{1RDM} & \multicolumn{1}{c}{$N-1$} & \multicolumn{1}{c}{$N+1$} \\
\hline
${}^1$P$_1$ & 0 & -167.5 & 0.00 & 0.00 & -22.57 \\
${}^1$P$_1$ & 1 &    0.0 & 0.00 & 0.00 &   0.00 \\
                               \hline\hline
\end{tabular}
\end{table}


\subsubsection{Wave function analysis for the $^{}1$P$_1$ state of beryllium}

With the 1s electrons frozen, the v2RDM-optimized 2RDM for the $M_J = 0$ projection of the $^1$P$_1$ state of beryllium is exactly ensemble $N$-representable but not pure-state $N$-representable. This property implies that the 2RDM is derivable from a sum of at least two pure-state 2RDMs. Interestingly, this example is simple enough for us to deduce numerically a set of two-electron wave functions whose 2RDMs can be combined to yield the ensemble $N$-representable 2RDM we obtain from v2RDM theory.

For this state, we expand all quantities in the basis of real-valued Hartree-Fock orbitals for the ground state (${}^1$S$_0$). The 1s orbital is frozen at double occupation, and the 2s, 2p$_x$, 2p$_y$, and 2p$_z$ orbitals are active.
In this basis, the 1RDM is diagonal with the $\alpha$- and $\beta$-spin blocks being equivalent ($^1D^{\alpha}_{\alpha}$ = $^1D^{\beta}_{\beta}$), and the only non-zero elements of the 2RDM arise in the $\alpha\beta$-spin block ($^2D^{\alpha\beta}_{\alpha\beta}$). Moreover, the  $^2D^{\alpha\beta}_{\alpha\beta}$ block has a special structure; the only non-zero elements are of the form ${}^2D^{i_\alpha i_\beta}_{j_\alpha j_\beta}$.  \textcolor{black}{This structure is a special case of a seniority-zero 2RDM, and it implies that the simplest form of underlying wave functions that define the ensemble must also have seniority-zero structure, \textit{i.e.} only determinants with all electrons paired comprise the wave function expansions. Although one can always find ensembles made of more complicated pure state wave function, we seek wave functions of the form}
\begin{eqnarray}
    \label{EQN:WFN}
    |\Psi \rangle &=& c_0 | 1s^2 2s^2 \rangle + c_1 | 1s^2 2p_x^2 \rangle \nonumber \\
    &+& c_2 | 1s^2 2p_y^2 \rangle+ c_3 | 1s^2 2p_z^2 \rangle
\end{eqnarray}
where $| 1s^2 2s^2 \rangle$ indicates a determinant of doubly occupied 1s and 2s orbitals.

Numerical analysis indicates that no single wave function of the form of Eq.~\ref{EQN:WFN} can yield the 2RDM obtained from our v2RDM calculations, but two wave functions, $|\Psi_1\rangle$ and $|\Psi_2\rangle$,
can as
\begin{eqnarray}
    {}^2D^{pq}_{rs} &=& 0.588 \langle \Psi_1| \hat{a}^\dagger_p \hat{a}^\dagger_q \hat{a}_s \hat{a}_r |\Psi_1 \rangle \nonumber \\
    &+& 0.412 \langle \Psi_2 |\hat{a}^\dagger_p \hat{a}^\dagger_q \hat{a}_s \hat{a}_r |\Psi_2 \rangle.
\end{eqnarray}
The expansion coefficients that define $|\Psi_1\rangle$ and $|\Psi_2\rangle$ are provided in Table \ref{TABLE:WFN_COEFS}.
What is interesting here is that neither $|\Psi_1\rangle$ nor $|\Psi_2\rangle$ are  eigenfunctions $\hat{L}^2$ (see Table \ref{TABLE:WFN_COEFS}), whereas the expectation value of this operator is constrained within the v2RDM calculation. Indeed, we can see that the ensemble 2RDM generated from these wave functions does have the correct value for $L(L+1)$, \textit{i.e.}, $1.378 \times 0.588 + 2.890 \times 0.412 \approx 2$. Hence, it appears that the low energy from v2RDM theory derives from the fact that the ensemble that defines the 2RDM does not have a good orbital angular momentum quantum number. Perhaps constraints on the variance of $\hat{L}^2$ could rectify this situation, but this quantity depends on the four-particle RDM and would thus be challenging to constrain in practice.



\begin{table}[]
\centering
\caption{Wave function expansion coefficients for two wave functions whose 2RDMs map onto the v2RDM-generated ensemble 2RDM for $M_J = 0$ $^1P_1$ of Be. The expectation value of $\hat{L}^2$ is also provided for these two wave functions.}
\label{TABLE:WFN_COEFS}
\begin{tabular}{cdd}
\hline
\hline
 & \multicolumn{1}{c}{$|\Psi_1 \rangle$} & \multicolumn{1}{c}{$|\Psi_2 \rangle$}\\
 \hline
  $c_0$ & -0.831 & -0.681 \\
  $c_1$ &  0.359 & -0.149 \\
  $c_2$ &  0.359 & -0.149 \\
  $c_3$ & -0.228 &  0.701 \\
  \hline
  $\langle \hat{L}^2 \rangle$ & 1.377 & 2.890 \\

                              \hline\hline
\end{tabular}
\end{table}

\subsubsection{Generalized Pauli constraints for other atomic systems}

Lastly, we consider the relationship between energy errors and GPC errors for v2RDM-optimized total angular momentum states in two additional atomic systems, boron and carbon, as described by v2RDM theory under PQG conditions and within the STO-3G basis set. With all electrons correlated among all orbitals, wave functions for these systems belong to the $\wedge^5\mathcal{H}_{10}$ and $\wedge^6\mathcal{H}_{10}$ families, respectively. Note, however, that we actually apply GPCs to the one-hole RDM of carbon, and that these conditions are equivalent to those of $\wedge^4\mathcal{H}_{10}$ wave functions. For GPCs applied to the 2RDM, we consider here only the ($N-1$)-electron states that belong to the $\wedge^4\mathcal{H}_{10}$ and $\wedge^5\mathcal{H}_{10}$ families in the case of boron and carbon, respectively.

Table \ref{TABLE:GPC} provides energy and GPC errors for v2RDM-optimized total angular momentum states in boron and carbon. One notable observation is that the GPCs on the 1RDM are satisfied for all states, regardless of the observed energy error. This result stands in stark contrast to those of Ref.~\citenum{DePrince16_164109}, where 1RDMs optimized without any orbital or total angular momentum constraints displayed large errors in GPCs for the ground states of boron (${}^2$P) and carbon (${}^3$P). So, it seems that the application of angular momentum constraints leads to pure-state 1RDMs, at least for the systems we have presented. Beyond this success, we find that GPCs on the 2RDM are violated for all cases that exhibit non-zero energy error, but, curiously, the magnitudes of the GPC errors do not correlate well with the magnitudes of the energy errors. For example, the absolute energy error of the $M_J = 0$ projection of the ${}^3$D$_2$ state of carbon is 37 times larger than that for the $M_J = 0$ projection of the ${}^3$P$_1$ state, and, yet, the error in the GPCs on the 2RDM is 19 times larger for the latter state. Lastly, we note that one of the states with zero energy error, the $M_J = 3$ projection of the ${}^3$D$_3$ state of carbon, is a Hartree-Fock state. The optimized 1RDM is idempotent, and the 2RDM is simply an antisymmetrized product of the 1RDM with itself, as expected, and thus both the 1RDM and 2RDM are exactly pure-state $N$-representable.

\begin{table}[]
\centering
\caption{Energy errors (10$^{-3}$ E$_{\rm h}$) and GPC errors for v2RDM-optimized total angular momentum states in boron and carbon atoms.}
\label{TABLE:GPC}
\begin{tabular}{cccddd}
\hline
\hline
& & & & \multicolumn{2}{c}{GPC errors} \\
\cline{5-6}
                              &             & J$_z$  & \multicolumn{1}{c}{energy error} & \multicolumn{1}{c}{1RDM} & \multicolumn{1}{c}{2RDM} \\ 
                              \hline 

 \multirow{3}{*}{B}     &  $^2P_{1/2}$ & 	1/2 & 	-0.6 &   0.00 & -188.78 \\
  & $^2P_{3/2}$	 & 1/2 & 	-2.9	 &   0.00 & -353.55 \\
 & $^2P_{3/2}$ & 	3/2 & 	0.0	 &   0.00 & 0.00 \\

                              \hline
  \multirow{15}{*}{C}    & 	$^3P_0$	 & 0     &   -3.7 &   0.00 & 	  -1.28 \\
                         &	$^3P_1$  & 0	 &   -4.5 &   0.00 & 	-186.31 \\
                         &	$^3P_1$	 & 1	 &   -1.3 &   0.00 &       -1.93 \\
                         &	$^3P_2$	 & 0	 &   -4.4 &   0.00 & 	 -10.39 \\
                         &	$^3P_2$	 & 1	 &   -1.4 &   0.00 & 	  -2.08 \\
                         &	$^3P_2$	 & 2	 &   0.0 &   0.00 & 	 -28.80 \\
                         &	$^3D_1$	 & 0	 & -131.7 &   0.00 & 	  -7.77 \\
                         &	$^3D_1$	 & 1	 &  -13.6 &   0.00 & 	 -20.77 \\
                         &	$^3D_2$	 & 0	 & -168.0 &   0.00 & 	  -9.79 \\
                         &	$^3D_2$	 & 1	 & -126.7 &   0.00 & 	 -45.86 \\
                         &	$^3D_2$	 & 2     &   0.0 &   0.00 & 	   0.00 \\
                         &	$^3D_3$	 & 0	 & -107.8 &   0.00 & 	  -6.45 \\
                         &	$^3D_3$	 & 1	 &  -28.5 &   0.00 & 	 -36.01 \\
                         &	$^3D_3$	 & 2	 &   0.0 &   0.00 & 	   0.00 \\
                         &	$^3D_3$	 & 3	 &   0.0 &   0.00 & 	   0.00 \\

                              \hline
                              \hline
\end{tabular}
\end{table}


